APT: Adaptive Pruning and Tuning Pretrained Language Models for Efficient Training and Inference

Fine-tuning and inference with large Language Models (LM) are generally known to be expensive. Parameter-efficient fine-tuning over pretrained LMs reduces training memory by updating a small number of LM parameters but does not improve inference efficiency. Structured pruning improves LM inference efficiency by removing consistent parameter blocks, yet often increases training memory and time. To improve both training and inference efficiency, we introduce APT that adaptively prunes and tunes parameters for the LMs. At the early stage of fine-tuning, APT dynamically adds salient tuning parameters for fast and accurate convergence while discarding unimportant parameters for efficiency. Compared to baselines, our experiments show that APT maintains up to 98% task performance when pruning RoBERTa and T5 models with 40% parameters left while keeping 86.4% LLaMA models' performance with 70% parameters remained. Furthermore, APT speeds up LMs fine-tuning by up to 8x and reduces large LMs memory training footprint by up to 70%.

==> sections/acknowledgements.tex <==
\section*{Acknowledgements}

==> tables/ablate_elastic.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[htbp]
% \begin{table}[]
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{@{}l|rr|rr@{}}
\toprule
Method                                    & SST2 & MNLI & Train Speed($\Uparrow$) & Train Mem($\Downarrow$) \\ \midrule
\ourmethod                                & 94.5 & 86.4 & 16.9\%       & 70.1\%        \\
\tableindent w/o $\mathcal{A}_{\text{P}}$ & 94.4 & 87.5 & 121.0\%      & 62.2\%        \\
\tableindent w/o salience                 & 94.3 & 84.7 & 16.4\%       & 65.0\%        \\
\tableindent w/o $\mathcal{A}_{\text{T}}$ & 93.2 & 84.5 & 14.6\%       & 64.4\%        \\
\tableindent w/o $\mathcal{D}_{\text{S}}$ & 92.9 & 85.3 & 20.7\%       & 61.9\%        \\ \bottomrule
\end{tabular}
}
\caption{Results of ablating salience-based allocation strategy and {\ourarch} with RoBERTa-base model, with relative training efficiency metrics to fine-tuning.}
\label{tab:ablate-paramalloc}
\vspace{-5pt}
\end{table}

==> tables/ablate_pruning.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{l|ll}
\hline
Pruning Metric & \multicolumn{1}{r}{MNLI} & \multicolumn{1}{r}{SQuAD} \\ \hline
\ourmethod &  &  \\
\tableindent w/o cross-info &  &  \\
\tableindent w/o cross-arrange &  &  \\
Salience &  &  \\
Magnitude &  &  \\ \hline
\end{tabular}
\caption{Results for replacing our proposed layer-wise fisher pruning objective with other metrics, including in-layer only fisher information, cross-information but without cross-layer rearrangement, salience (weight-gradient product), and magnitude}
\label{tab:ablate-pruning}
\end{table}

==> tables/bert_main_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t!]
\centering
\begin{tabular}{@{}ll|rrr|rrrr@{}}
\toprule
Tune & Prune & SST-2 & MNLI & SQuAD & Train $\nearrow$ & Train Mem. & Inf. $\nearrow$ & Inf. Mem \\ \midrule
FT & None & 93.5 & 84.6 & 88.5 & 1.00$\times$ & 100\% & 1.00$\times$ & 100\% \\
FT & CoFi & 93.0 & 85.3 & 89.1 & 0.67$\times$ & 162\% &  &  \\
FT & MT &  & 68.1 &  & 1.00$\times$ & 100\% &  &  \\
FT & MT* &  &  &  &  &  &  &  \\ \midrule
LoRA & None & 92.9 & 84.2 & 83.5 & 1.16$\times$ &  & 1.00$\times$  & 100\% \\
LoRA & CoFi &  &  &  & &  &   &  \\
LoRA & MT &  & 31.8 & & 1.16$\times$ & 80.5\% &  &  \\ 
LoRA & MT* &  & & & &  &  &  \\ \midrule
\begin{tabular}[c]{@{}l@{}}\ourmethod\\ \tableindent w/o Distillation\end{tabular} &  & 91.5 & 80 & 75.3 & 1.31$\times$ & 77.94\% & 2.16$\times$ & 51.3\% \\
\ourmethod &  & 92.4 &  & 87.0 &  &  &  &  \\ \bottomrule
\end{tabular}
\caption{The main results of \ourmethod compared with baselines on $\text{BERT}_{\text{BASE}}$ backbone given 40\% tuned model FLOP constraint with the tuning parameter number less than 2.5M. Train $\nearrow$ denotes the average training speed per epoch compared to fine-tuning. Train Mem. denotes the peak memory consumption throughout training. Inf. $\nearrow$ and Inf. Mem denotes the inference time speedup and memory usage compared with the vanilla fine-tuned model. FT denotes fully fine-tuning. MT denotes Mask Tuning, while MT* denotes retraining after Mask Tuning.}
\label{tab:main-result}
\end{table*}

==> tables/llama_2_13b_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[htbp]
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
Method    & Target Density & Init Density & T. M.   & ARC   & HellaSWAG & MMLU  & TruthfulQA & Avg.    \\ \midrule
None      & 100\%           & 100\%         & 100\%    & 59.39 & 82.13     & 55.77 & 37.38      & 58.6675 \\
LoRA      & 100\%           & 100\%         & 100\%    & 60.84 & 82.82     & 55.95 & 46.5       & 61.5275 \\ \midrule
LoRA + $\text{MT}_{\text{train}}$ & 70\%            & 70\%          & 100\%    & 56.4  & 79.08     & 50.71 & 42.07      & 57.065  \\
LLMPruner & 70\%            & 70\%          &         &       &           &       &            &         \\
APT       & 70\%            & 100\%         & 100.50\% & 45.9  &           &       & 47.37      &         \\
APT       & 70\%            & 85\%          & 86.24\%  & 47.95 & 75.61     & 50.28 & 46.33      & 55.0425 \\
APT       & 70\%            & 70\%          & 75.82\%  & 49.49 & 75.84     & 52.46 & 44.67      & 55.615  \\ \midrule
LoRA + $\text{MT}_{\text{train}}$ & 50\%            & 50\%          & 100\%    & 38.4  & 60.55     & 42.92 & 46.51      & 47.095  \\
LLMPruner & 50\%            & 50\%          &         &       &           &       &            &         \\
APT       & 50\%            & 100\%         &         &       &           &       &            &         \\
APT       & 50\%            & 75\%          & 78.03\%  & 36.86 & 57.15     &       & 41.54      &         \\
APT       & 50\%            & 50\%          &         & 36.35 & 55        & 30.71 & 45.44      & 41.875  \\ \bottomrule
\end{tabular}
\caption{Main results of {\ourmethod} compared to structured pruning baselines on LLaMA 2 13B model.}
\label{tab:llama-2-13b-main-result}
\end{table*}

==> tables/llama_7b_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{@{}l|llrrr|llll@{}}
\toprule
Method       & ARC                            & HellaSwag                      & MMLU                           & TruthfulQA                     & Avg.                           & Train Speed($\Uparrow$) & Train Mem ($\Downarrow$) & Inf Speed($\Uparrow$) & Inf Mem($\Downarrow$) \\ \midrule
LLaMA 2 7B   & 53.1                           & 77.7                           & 43.8                           & 39.0                           & 53.4                           & -            & -           & -          & -         \\ 
LoRA         & 55.6                           & 79.3                           & 46.9                           & 49.9                           & 57.9                           & 100.0\%      & 100.0\%     & 100.0\%    & 100.0\%   \\ \midrule
LoRA+Prune & \textbf{46.8} & 65.2                           & 23.9                           & 46.2                           & 45.5                           & 55.3\%       & 100.0\%     & 115.5\%    & 68.9\%    \\
LLMPruner    & 39.2                           & 67.0                           & 24.9                           & 40.6                           & 42.9                           & 115.1\%      & 253.6\%     & 114.8\%    & 74.2\%    \\
APT          & 45.4                           & \textbf{71.1} & \textbf{36.9} & \textbf{46.6} & \textbf{50.0} & 94.3\%       & 75.8\%      & 117.0\%    & 67.2\%    \\ \bottomrule
\end{tabular}
}
\caption{
% \hanna{this table has a different set of baelines, explain why you are using a diferent baseline here. }
    LLaMA 2 7B 30\% sparsity pruning results with GPT4-generated Alpaca dataset, evaluated on the Open LLM leaderboard few-shot tasks. Training speed is measured via training time per step. We do not compare to distillation baselines because the training cost of distillation is too large, and we also compare {\ourmethod} to LLMPruner since it is dedicated to large {\lmabbr} pruning. $\Uparrow$ denotes the metric is better when bigger, and $\Downarrow$ denotes smaller is better.}
\label{tab:llama-7b-results}
\vspace{-15pt}
\end{table*}

==> tables/merged_main_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t!]
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{@{}ll|rrrr|rrrr@{}}
\toprule
Model                                           & Method         & MNLI          & SST2          & SQuAD v2      & CNN/DM                  & Train Speed($\Uparrow$) & Train Mem($\Downarrow$) & Inf Speed($\Uparrow$) & Inf Mem($\Downarrow$) \\ \midrule
\multirow{5}{*}{$\text{RoBERTa}_{\text{base}}$} & FT             & 87.6          & 94.8          & 82.9          & -                       & 100.0\%      & 100.0\%     & 100.0\%    & 100.0\%   \\
                                                & LoRA           & 87.5          & 95.1          & 83.0          & -                       & 4.7\%        & 60.5\%      & 100.0\%    & 100.0\%   \\ \cmidrule(l){2-10} 
                                                & LoRA+Prune   & 84.0          & 93.0          & 79.2          & -                       & 2.0\%        & 60.5\%      & 262.9\%    & 75.1\%    \\
                                                & Prune+Distill   & \textbf{87.3}          & \textbf{94.5}          &   -        & -                       & 6.7\%        & 168.5\%      & 259.2\%    & 79.2\%    \\
                                                & LoRA+Prune+Distill & 84.2          & 91.9          & -             & -                       & 1.5\%        & 141.4\%     & 253.7\%    & 82.3\%    \\ \cmidrule(l){2-10} 
                                                & \ourmethod     & 86.4 & \textbf{94.5} & \textbf{81.8} & -                       & 16.9\%       & 70.1\%      & 241.9\%    & 78.1\%    \\ \midrule
\multirow{4}{*}{$\text{T5}_{\text{base}}$}      & FT             & 87.1          & 95.2          & -             & 42.1/20.3/39.4          & 100.0\%      & 100.0\%     & 100.0\%    & 100.0\%   \\
                                                & LoRA           & 87.0          & 95.0          & -             & 38.7/17.2/36.0          & 39.1\%       & 62.0\%      & 100.0\%    & 100.0\%   \\
                                                & LoRA+Prune   & 80.9          & 92.3          & -             & 36.7/15.7/33.9          & 2.5\%        & 62.0\%      & 212.5\%    & 73.4\%    \\ \cmidrule(l){2-10} 
                                                & \ourmethod     & \textbf{87.0} & \textbf{95.0} & -             & \textbf{38.6/17.0/35.8} & 20.6\%       & 73.9\%      & 134.1\%    & 81.5\%    \\ \bottomrule
\end{tabular}
}
\caption{RoBERTa and T5 pruning with {\ourmethod} compared to baselines under 60\% sparsity. We measure the training and inference efficiency with {\lmabbr}s pruned on the SST2 task. Training speed is measured via 97\% accuracy TTA. $\Uparrow$ denotes the metric is better when bigger, and $\Downarrow$ denotes smaller is better.}
\label{tab:small-model-results}
\vspace{-5pt}
\end{table*}

==> tables/roberta_main_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{wraptable}{l}{0.6\textwidth}
\begin{table*}[htbp]
\begin{tabular}{@{}l|lrr|llll@{}}
\toprule
Method                    & MNLI                           & SST2                           & SQuAD v2                       & Train. Speed & Train. Mem. & Inf. Speed & Inf. Mem. \\ \midrule
FT                        & 87.6                           & 94.8                           & 82.9                           & 100.0\%      & 100.0\%     & 100.0\%    & 100.0\%   \\
LoRA                      & 87.5                           & 95.1                           & 83.0                           & 4.7\%        & 60.5\%      & 100.0\%    & 100.0\%   \\ \midrule
LoRA + Prune              & 84.0                           & 93.0                           & 79.2                           & 2.0\%        & 60.5\%      & 262.9\%    & 75.1\%    \\
LoRA + Distill            & 84.2                           & 91.9                           & -                              & 1.5\%        & 141.4\%     & 253.7\%    & 82.3\%    \\ \midrule
\ourmethod & \textbf{86.4} & \textbf{94.5} & \textbf{81.8} & 16.9\%       & 70.1\%      & 241.9\%      & 78.1\%    \\ \bottomrule
\end{tabular}
\caption{RoBERTa pruning with {\ourmethod} compared to baselines under 60\% sparsity. We measure the training and inference efficiency with {\lmabbr}s pruned on the SST2 task. Training speed is measured via 97\% accuracy TTA.}
\label{tab:main-result}
% \vspace{-15pt}
\end{table*}

==> tables/roberta_sst2_training_efficiency.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[htbp]
\centering
\begin{tabular}{@{}lr|rrrrrr@{}}
\toprule
Method                         & Density & SST2 & 97\% TTA     & 99\% TTA     & T. M. & Inf. $\nearrow$ & Inf. Mem. \\ \midrule
FT                             & 100\%   & 94.8 & 1.00$\times$ & 1.00$\times$ & 100\%           & 1.00$\times$ & 100.0\%  \\
LoRA                           & 100\%    & 95.1 & 21.4$\times$ & 8.39$\times$ & 60.5\%          & 1.00$\times$ & 100.0\%  \\ \midrule
FT + $\text{MT}_{\text{train}}$              & 40\%    & 93.5 & 6.80$\times$ & -            & 100\%           & 2.67$\times$ & 76.4\%   \\
LoRA + $\text{MT}_{\text{train}}$            & 40\%    & 93.0   & 51.3$\times$ & -            & 60.5\%          & 2.63$\times$ & 75.1\%   \\
% LoRA* + $\text{MT}_{\text{train}}$ & 40\%    & 93.2 & 51.3$\times$ & -            & 60.5\%          & 2.57$\times$ & 74.2\%   \\
FT + $\text{MT}_{\text{distill}}$              & 40\%    & 94.3 & 9.40$\times$ & 6.17$\times$ & 100\%           & 2.60$\times$ & 76.4\%   \\
LoRA + $\text{MT}_{\text{distill}}$            & 40\%    & 92.3 & 65.3$\times$ & -            & 70.5\%          & 2.60$\times$ & 75.1\%   \\
% LoRA* + $\text{MT}_{\text{distill}}$ & 40\%    & 92.8 & 65.3$\times$ & -            & 70.5\%          & 2.60$\times$ & 75.1\%   \\
FT + CoFi                      & 40\%    & 94.5 & 15.0$\times$ & -            & 168.5\%         & 2.59$\times$ & 79.2\%   \\
LoRA + CoFi                    & 40\%    & 91.9 & 65.3$\times$ & -            & 141.4\%         & 2.54$\times$ & 82.3\%   \\ \midrule
{\ourmethod}                  & 40\%    & 94.5 & 5.92$\times$ & 4.13$\times$ & 62.7\%          & 2.71$\times$ & 79.5\%   \\ \bottomrule
\end{tabular}
\caption{RoBERTa-base SST2 performance and efficiency results. LoRA* denotes the setting where we use the model tuned with LoRA after the same amount of epochs when fine-tuning converges as the trained/teacher model. T.M. denotes the relative training peak memory to full fine-tuning. Inf. $\nearrow$ and Inf. Mem. represent the relative inference speedup and memory usage compared to full fine-tuning.}
\label{tab:roberta-base-sst2}
\end{table*}

==> tables/t5_3b_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lr|rrrr@{}}
\toprule
Method                         & Density & SST2 & CNN/DM &  T. M. & Inf. Speedup \\ \midrule
FT                           & 100\%   & 97.4 &  42.72/21.02/39.94  &            &              \\
LoRA                           & 100\%   & 97.5 &        &            &              \\ \midrule
LoRA + $\text{MT}_{\text{train}}$            & 8\%    &   83.1  &         &       &              \\
LoRA + $\text{MT}_{\text{distill}}$            & 8\%    & 90.9  &           &       &              \\
{\ourmethod}                  & 8\%    &  92.0  &        &          &              \\ \bottomrule
\end{tabular}
\caption{T5-XL results}
\label{tab:t5-3b-results}
\end{table}

==> tables/t5_main_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[htbp]
\centering
\begin{tabular}{@{}l|rlr|llll@{}}
\toprule
Method                        & MNLI                           & SST2                           & CNN/DM                                                                                       & Train. Speed & Train. Mem. & Inf. Speed & Inf. Mem. \\ \midrule
FT                            & 87.1                           & 95.2                           & 42.1/20.3/39.4                                                                               & 100.0\%      & 100.0\%     & 100.0\%    & 100.0\%   \\
LoRA                          & 87.0                           & 95.0                           & 38.7/17.2/36.0                                                                               & 39.1\%       & 62.0\%      & 100.0\%    & 100.0\%   \\ \midrule
LoRA + Prune                  & 80.9                           & 92.3                           & 36.7/15.7/33.9                                                                               & 2.5\%        & 62.0\%      & 212.5\%    & 73.4\%    \\ \midrule
{\ourmethod} & \textbf{87.0} & \textbf{95.0} & \textbf{38.6}/\textbf{17.0}/\textbf{35.8} & 20.6\%       & 73.9\%      & 134.1\%    & 81.5\%    \\ \bottomrule
\end{tabular}
\caption{T5 model pruning with {\ourmethod} compared to existing baselines under 60\% sparsity. We measure the training and inference efficiency with {\lmabbr}s pruned on the SST2 task. Training speed is measured via 97\% accuracy TTA.}
\label{tab:t5-main-results}
\vspace{-15pt}
\end{table*}

==> tables/t5_wmt_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lr|rrrrr@{}}
\toprule
Method                         & Density & CNN/DM & 97\% TTA & T. M. & Inf. Speedup & Inf. Mem \\ \midrule
FT                             & 100\%   &  42.05/20.34/39.40 & 1.00$\times$ & 100.0\%   & 1.00$\times$    & 100.0\%  \\
LoRA                           & 100\%   &           &    &   81.6\%    &  1.00$\times$    & 100.0\%         \\ \midrule
FT + $\text{MT}_{\text{train}}$              & 40\%    &           &          &                 &              &          \\
LoRA + $\text{MT}_{\text{train}}$            & 40\%    &           &          &                 &              &          \\
LoRA* + $\text{MT}_{\text{train}}$ & 40\%    &           &          &                 &              &          \\
FT + $\text{MT}_{\text{distill}}$              & 40\%    &           &          &                 &              &          \\
LoRA + $\text{MT}_{\text{distill}}$            & 40\%    &           &          &                 &              &          \\
LoRA * + $\text{MT}_{\text{distill}}$ & 40\%    &           &          &                 &              &          \\ \midrule
{\ourmethod}                  & 40\%    &           &          &                 &              &          \\ \bottomrule
\end{tabular}
\caption{T5-base CNN/DM}
\label{tab:t5-base}
\end{table}
